ADVENT: Adversarial Entropy Minimization for Domain Adaptation in Semantic Segmentation

Semantic segmentation is a key problem for many computer vision tasks. While approaches based on convolutional neural networks constantly break new records on different benchmarks, generalizing well to diverse testing environments remains a major challenge. In numerous real world applications, there is indeed a large gap between data distributions in train and test domains, which results in severe performance loss at run-time. In this work, we address the task of unsupervised domain adaptation in semantic segmentation with losses based on the entropy of the pixel-wise predictions. To this end, we propose two novel, complementary methods using (i) entropy loss and (ii) adversarial loss respectively. We demonstrate state-of-the-art performance in semantic segmentation on two challenging "synthetic-2-real" set-ups and show that the approach can also be used for detection.

==> qualres.tex <==
Figure~\ref{fig:sup_qual_det} and Figure~\ref{fig:sup_qual_seg} illustrate qualitative results for object detection and semantic segmentation.

\begin{figure*}[th!]
	%\captionsetup[subfigure]{labelformat=empty}
	\begin{center}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\caption{Input image}\vspace{-0.2cm}
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/164_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\caption{Without adaptation}\vspace{-0.2cm}
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/164_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\caption{MinEnt}\vspace{-0.2cm}
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/164_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\caption{AdvEnt}\vspace{-0.2cm}
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/164_image.png}
		\end{subfigure}\\\vspace{0.1cm}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/165_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/165_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/165_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/165_image.png}
		\end{subfigure}\\\vspace{0.1cm}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/172_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/172_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/172_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/172_image.png}
		\end{subfigure}\\\vspace{0.1cm}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/174_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/174_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/174_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/174_image.png}
		\end{subfigure}\\\vspace{0.1cm}
		%		\begin{subfigure}[t]{0.24\textwidth}\centering
		%			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/182_image.png}
		%		\end{subfigure}
		%		\begin{subfigure}[t]{0.24\textwidth}\centering
		%			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/182_image.png}
		%		\end{subfigure}
		%		\begin{subfigure}[t]{0.24\textwidth}\centering
		%			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/182_image.png}
		%		\end{subfigure}
		%		\begin{subfigure}[t]{0.24\textwidth}\centering
		%			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/182_image.png}
		%		\end{subfigure}\\\vspace{0.1cm}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/203_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/203_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/203_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/203_image.png}
		\end{subfigure}\\\vspace{0.1cm}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/225_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/225_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/225_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/225_image.png}
		\end{subfigure}\\\vspace{0.1cm}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/241_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/241_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/241_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/241_image.png}
		\end{subfigure}\\\vspace{0.1cm}
%		\begin{subfigure}[t]{0.24\textwidth}\centering
%			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/267_image.png}
%		\end{subfigure}
%		\begin{subfigure}[t]{0.24\textwidth}\centering
%			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/267_image.png}
%		\end{subfigure}
%		\begin{subfigure}[t]{0.24\textwidth}\centering
%			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/267_image.png}
%		\end{subfigure}
%		\begin{subfigure}[t]{0.24\textwidth}\centering
%			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/267_image.png}
%		\end{subfigure}\\\vspace{0.1cm}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/293_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/293_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/293_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/293_image.png}
		\end{subfigure}\\\vspace{0.1cm}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/raw-detection_result/294_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/baseline-detection_result/294_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/e-detection_result/294_image.png}
		\end{subfigure}
		\begin{subfigure}[t]{0.24\textwidth}\centering
			\includegraphics[width=.98\textwidth, trim={32mm 77mm 26mm 80mm}, clip]{./detection/adv-detection_result/294_image.png}
		\end{subfigure}\\\vspace{0.1cm}
	\end{center}
	\vspace{-0.3cm}
	\caption{\small Qualitative results for object detection. Column (a) shows the input images. Columns (b), (c) and (d) illustrate detection results of the baseline, our MinEnt and AdvEnt models. Detections of different classes are plotted in different colors. To produce the detections, we used a fixed threshold of $0.5$.}
	\vspace{-0.4cm}
	\label{fig:sup_qual_det}
\end{figure*}

\begin{figure*}[h]
	%\captionsetup[subfigure]{labelformat=empty}
	\begin{center}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\caption{Input image + GT}\vspace{-0.2cm}
					\includegraphics[width=.98\textwidth]{./results_qualitative_small/munster_000101_000019_leftImg8bit.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\caption{Without adaptation}\vspace{-0.2cm}
					\includegraphics[width=.98\textwidth]{./results_qualitative_small/munster_000101_000019_leftImg8bit_ent_onlysource.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\caption{MinEnt}\vspace{-0.2cm}
					\includegraphics[width=.98\textwidth]{./results_qualitative_small/munster_000101_000019_leftImg8bit_ent_entropy.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\caption{AdvEnt}\vspace{-0.2cm}
					\includegraphics[width=.98\textwidth]{./results_qualitative_small/munster_000101_000019_leftImg8bit_ent_advent.png}
				\end{subfigure}\\\vspace{0.1cm}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small/munster_000101_000019_color.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small/munster_000101_000019_leftImg8bit_onlysource.jpg}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small/munster_000101_000019_leftImg8bit_entropy.jpg}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small/munster_000101_000019_leftImg8bit_advent.jpg}
				\end{subfigure}\\\vspace{-0.13cm}
				\hdashrule[1ex][x]{17cm}{1.5pt}{1.5mm}\vspace{-0.13cm}
				\begin{subfigure}[t]{0.24\textwidth}\centering
%					\caption{Input image + GT}\vspace{-0.2cm}
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000158_000019_leftImg8bit.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
%					\caption{Without adaptation}\vspace{-0.2cm}
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000158_000019_leftImg8bit_ent_onlysource.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
%					\caption{MinEnt}\vspace{-0.2cm}
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000158_000019_leftImg8bit_ent_entropy.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
%					\caption{AdvEnt}\vspace{-0.2cm}
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000158_000019_leftImg8bit_ent_advent.png}
				\end{subfigure}\\\vspace{0.1cm}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000158_000019_color.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000158_000019_leftImg8bit_onlysource.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000158_000019_leftImg8bit_entropy.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000158_000019_leftImg8bit_advent.png}
				\end{subfigure}\\\vspace{-0.13cm}
				\hdashrule[1ex][x]{17cm}{1.5pt}{1.5mm}\vspace{-0.13cm}
				%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000169_000019_leftImg8bit.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000169_000019_leftImg8bit_ent_onlysource.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000169_000019_leftImg8bit_ent_entropy.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000169_000019_leftImg8bit_ent_advent.png}
				\end{subfigure}\\\vspace{0.1cm}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000169_000019_color.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000169_000019_leftImg8bit_onlysource.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000169_000019_leftImg8bit_entropy.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000169_000019_leftImg8bit_advent.png}
				\end{subfigure}\\\vspace{-0.13cm}
				\hdashrule[1ex][x]{17cm}{1.5pt}{1.5mm}\vspace{-0.13cm}
				%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000016_000019_leftImg8bit.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000016_000019_leftImg8bit_ent_onlysource.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000016_000019_leftImg8bit_ent_entropy.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000016_000019_leftImg8bit_ent_advent.png}
				\end{subfigure}\\\vspace{0.1cm}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000016_000019_color.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000016_000019_leftImg8bit_onlysource.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000016_000019_leftImg8bit_entropy.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000016_000019_leftImg8bit_advent.png}
				\end{subfigure}\\\vspace{-0.13cm}
				\hdashrule[1ex][x]{17cm}{1.5pt}{1.5mm}\vspace{-0.13cm}
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000129_000019_leftImg8bit.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000129_000019_leftImg8bit_ent_onlysource.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000129_000019_leftImg8bit_ent_entropy.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000129_000019_leftImg8bit_ent_advent.png}
				\end{subfigure}\\\vspace{0.1cm}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000129_000019_color.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000129_000019_leftImg8bit_onlysource.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000129_000019_leftImg8bit_entropy.png}
				\end{subfigure}
				\begin{subfigure}[t]{0.24\textwidth}\centering
					\includegraphics[width=.98\textwidth]{./results_qualitative_small_local/munster_000129_000019_leftImg8bit_advent.png}
				\end{subfigure}
				%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\end{center}
	\vspace{-0.3cm}
	\caption{\small Qualitative results of semantic segmentation. Column (a) shows input images and the corresponding semantic segmentation ground-truths. Column (b), (c) and (d) show segmentation results (upper) along with prediction entropy maps produced by different approaches (lower).}
	\vspace{-0.4cm}
	\label{fig:sup_qual_seg}
\end{figure*}

